Beyond Clicking:A Step Towards Generalist GUI Grounding via Text Dragging

Graphical user interface (GUI) grounding, the process of mapping human instructions to GUI actions, serves as a fundamental basis to autonomous GUI agents. While existing grounding models achieve promising performance to simulate the mouse click action on various click-based benchmarks, another essential mode of mouse interaction, namely dragging, remains largely underexplored. Yet, dragging the mouse to select and manipulate textual content represents a prevalent and important usage in practical GUI scenarios. To narrow this gap, we first introduce GUI-Drag, a diverse dataset of 161K text dragging examples synthesized through a scalable pipeline. To support systematic and robust evaluation, we further construct ScreenDrag, a benchmark with 5,333 examples spanning three levels of interface context, together with three dedicated metrics designed for assessing text dragging capability. Models trained on GUI-Drag with an efficient continual training strategy achieve substantial improvements on ScreenDrag, while preserving the original click-based performance on ScreenSpot, ScreenSpot-v2, and OSWorld-G. Our work encourages further research on broader GUI grounding beyond just clicking and paves way toward a truly generalist GUI grounding model. All benchmark, data, checkpoints, and code are open-sourced and available at https://osu-nlp-group.github.io/GUI-Drag.

==> tables/results_backup.tex <==
\begin{table}[!hbp] \centering \small \caption{Performance on {\benchmark} with breakdown on text-sparse and text-dense settings. The best and second-best results under each metric are \textbf{bolded} and \underline{underlined}.} \vspace{0.5em} \label{tab:exp_text_density} \renewcommand{\arraystretch}{1.15} \setlength{\tabcolsep}{6pt} \begin{tabular}{l c cc cc cc} \toprule \multirow{2}{*}{\textbf{Experimental Setting}} & \multirow{2}{*}{\textbf{DTR$\uparrow$}} & \multicolumn{2}{c}{\textbf{Text-Sparse}} & \multicolumn{2}{c}{\textbf{Text-Dense}} & \multicolumn{2}{c}{\textbf{Avg.}} \\ \cmidrule(lr){3-4}\cmidrule(lr){5-6} & & \textbf{B-Dist$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{B-Dist$\downarrow$} & \textbf{SR$\uparrow$} \\ \midrule \multicolumn{6}{c}{\textbf{Open-Source}} \\ \midrule Qwen2.5-VL-3B & 5.0\% & 44.5 & 3.2\% & 43.8 & 0.0\% \\ Qwen2.5-VL-7B & 5.0\% & 27.7 & 3.3\% & 30.8 & 1.1\% \\ Qwen2.5-VL-32B & 55.8\% & 23.4 & 5.8\% & 27.0 & 1.6\% \\ Jedi-3B & 94.1\% & 12.1 & 19.0\%& 17.2 & 8.5\% \\ Jedi-7B & 77.5\% & 14.3 & 12.0\%& 18.3 & 4.9\% \\ UI-TARS-1.5-7B & 84.6\% & 13.0 & 23.6\%& 19.5 & 9.3\% \\ \midrule \multicolumn{6}{c}{\textbf{Closed-Source}} \\ \midrule OpenAI CUA & 85.7\% & 9.7 & 21.4\% & 12.8 & 8.1\% \\ Claude CUA & 47.4\% & 10.4 & 17.0\% & 8.9 & 12.5\% \\ OpenAI CUA (w/ hint) & 91.7\% & 8.6 & 18.0\% & 12.9 & 6.7\% \\ Claude CUA (w/ hint) & \underline{96.9}\% & 8.6 & 16.9\% & 10.7 & 11.3\% \\ \midrule \multicolumn{6}{c}{\textbf{Ours}} \\ \midrule Jedi-3B (Drag) & \textbf{100.0}\% & 7.9 & \underline{39.7}\% & 9.2 & \underline{20.1}\% \\ Jedi-7B (Drag) & \textbf{100.0}\% & 7.4 & 36.1\% & 8.8 & 16.6\% \\ {\model}-3B & \textbf{100.0}\% & \underline{6.9} & \textbf{43.6}\% & \underline{7.2} & \textbf{22.9}\% \\ {\model}-7B & \textbf{100.0}\% & \textbf{6.2} & 38.1\% & \textbf{6.7} & 19.8\% \\ \bottomrule \end{tabular} \end{table}
